A comprehensive approach to new physics simulations

We describe a framework to develop, implement and validate any perturbative Lagrangian-based particle physics model for further theoretical, phenomenological and experimental studies. The starting point is FeynRules, a Mathematica package that allows to generate Feynman rules for any Lagrangian and then, through dedicated interfaces, automatically pass the corresponding relevant information to any supported Monte Carlo event generator. We prove the power, robustness and flexibility of this approach by presenting a few examples of new physics models (the Hidden Abelian Higgs Model, the general Two-Higgs-Doublet Model, the most general Minimal Supersymmetric Standard Model, the Minimal Higgsless Model, Universal and Large Extra Dimensions, and QCD-inspired effective Lagrangians) and their implementation/validation in FeynArts/FormCalc, CalcHep, MadGraph/MadEvent, and Sherpa.

==> susy.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The most general Minimal Supersymmetric Standard Model}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Commands and definitions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\bpm{\begin{pmatrix}}
\def\epm{\end{pmatrix}}
\def\del{\partial}
\def\sdel{\slashed{\partial}}
\def\bsp#1\esp{\begin{split}#1\end{split}}
\def\hc{{\rm h.c.}}
\def\nn{\nonumber}
\def\cw{{\cos\theta_w}}
\def\cwd{{\cos^2\theta_w}}
\def\sw{{\sin\theta_w}}
\def\ca{{\cos\alpha}}
\def\sa{{\sin\alpha}}
\def\cb{{\cos\beta}}
\def\sb{{\sin\beta}}
\def\tb{{\tan\beta}}
\newcommand{\lag}{\begin{cal}L\end{cal}}
\newcommand{\doublet}[2]{\bpm#1\\#2\epm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Introduction}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Most present supersymmetric models are based on the four-dimensional supersymmetric field theory of Wess and Zumino \cite{Wess:1974tw}. The simplest model is the straightforward supersymmetrization of the Standard Model, with the same gauge interactions, including $R$-parity conservation, and is called the Minimal Supersymmetric Standard Model (MSSM) \cite{Nilles:1983ge, Haber:1984rc}. Its main features are to link bosons with fermions and unify internal and external symmetries. Moreover, it allows for a stabilization of the gap between the Planck and the electroweak scale and for gauge coupling unification at high energies, provides a dark matter candidate as the lightest supersymmetric particle and appears naturally in string theories. However, since supersymmetric particles have not yet been discovered, supersymmetry must be broken at low energies, which makes the superpartners massive in comparison to their Standard Model counterparts. 



Supersymmetric phenomenology at colliders has been extensively investigated for basic processes at leading order \cite{Dawson:1983fw, Craigie:1983as, Craigie:1984tk, Chiappetta:1985ku, delAguila:1990yw, Baer:1993ew, Gehrmann:2004xu, Bozzi:2004qq, Bozzi:2005sy, Bozzi:2007me, Fuks:2008ab, Debove:2008nr} and next-to-leading order \cite{Beenakker:1996ch, Beenakker:1997ut, Baer:1997nh, Berger:1998kh, Berger:1999mc, Berger:2000iu, Beenakker:1999xh} of perturbative QCD. More recently, for some processes, soft-gluon radiation has been resummed to all orders in the strong coupling constant and the results have been matched with the next-to-leading order calculations \cite{Bozzi:2006fw, Bozzi:2007qr, Bozzi:2007tea, Kulesza:2008jb, Debove:2009xx}. However, even if those calculations are useful for inclusive enough analyses, they are not suitable if we are interested in a proper description of the full collider environment, for which Monte-Carlo event generators are needed. For a couple of years, all the generators which we are interested in contain a built-in version of the MSSM. The model files for FeynArts/FormCalc are described in Ref.\ \cite{Hahn:2001rv, Hahn:2005qi}, for CalcHEP in Ref.\ \cite{Belanger:2004yn}, for MadGraph/MadEvent in Ref.\ \cite{Cho:2006sx}, and for SHERPA in Ref.\ \cite{Hagiwara:2005wg}. The SHERPA and FeynArts/FormCalc implementations keep generic mixing in the scalar sector while the other generators rely on a simplified model with only helicity-mixing for third generation sfermions.



Our MSSM implementation in FeynRules is the most general one in a sense that it is keeping all the flavour-violating and helicity-mixing terms in the Lagrangian and also all the possible additional CP-violating phases. This yields thus 105 new free parameters \cite{Dimopoulos:1995ju}, and in order to deal in a transparent way with all of those, our implementation will follow the commonly used universal set of conventions provided by the Supersymmetry Les Houches Accord (SLHA) \cite{Skands:2003cj, Allanach:2008qq}, except for some minor points. We will dedicate a complementary paper to a more complete description of the model \cite{Duhr:2009xx}.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{The implemented Lagrangian}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent{\textbf{Field content}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\arraystretch}{1.3}
\begin{table}[!h]
  \begin{center}
    \begin{tabular}{| c || c  c | c  c | c |}
      \hline Name & Particle & spin & Superpartner & spin &  Representations \\ 
      \hline\hline (s)quarks & $(\chi_{ui} \; \; \chi_{di} )^T$ & 1/2 & $(\tilde{u}^0_{Li} \;\; \tilde{d}^0_{Li} )^T$& 0 & $\big(\mathbf{3}, \mathbf{2},1/6\big)$\\ 
       & $\chi_{\bar ui}$ & 1/2 & $\tilde{u}^{0i\dagger}_R$ &0& $\big(\bar{\mathbf{3}}, \mathbf{1},-2/3 \big)$ \\
      & $\chi_{\bar di}$ & 1/2 & $\tilde{d}^{0i\dagger}_R$ &0& $\big(\bar{\mathbf{3}}, \mathbf{1},1/3 \big)$\\ 
      \hline (s)leptons & $(\chi_{\nu i} \; \; \chi_{li})^T$ &1/2 & $(\tilde{\nu}_i^0 \; \; \tilde{l}^0_{Li})^T$ & 0 & $\big(\mathbf{1}, \mathbf{2},-1/2 \big)$ \\
      & $\chi_{\bar li}$ & 1/2 & $\tilde{l}^{0i\dagger}_R$ &0& $\big(\mathbf{1}, \mathbf{1},1 \big)$ \\ 
      \hline Higgs(inos) & $(H_u^+\;\;H_u^0 )^T$ & 0 & $(\psi_{H_u^+}\, \, \psi_{H_u^0})^T$& 1/2 & $\big(\mathbf{1}, \mathbf{2}, 1/2\big)$\\
      & $(H_d^0\;\;H_d^- )^T$ & 0 & $(\psi_{H_d^0}\, \, \psi_{H_d^-})^T$& 1/2 & $\big(\mathbf{1}, \mathbf{2}, -1/2\big)$\\ 
      \hline $B$-boson, bino & $B^0$& 1 &$\psi_B$ & 1/2 &  $\big(\mathbf{1}, \mathbf{1}, 0\big)$\\
      $W$-bosons, winos & $(W^1 \; \; W^2 \; \;  W^3)^T$ & 1  &  $(\psi_{W^1} \; \; \psi_{W^2} \; \; \psi_{W^3})^T$ & 1/2 &  $\big(\mathbf{1}, \mathbf{3}, 0\big)$\\ 
      gluon, gluino & $g$& 1 &$\psi_g $ & 1/2 &  $\big(\mathbf{8}, \mathbf{1}, 0\big)$\\
      \hline 
    \end{tabular}
  \end{center} 
  \caption{\label{tab:MSSMFieldContent}The MSSM fields and their representations under the Standard Model gauge groups $SU(3)_C \times SU(2)_L \times U(1)_Y$. The quarks and leptons are denoted in terms of two-component Weyl spinors.}
\end{table}



Each of the Standard Model quark and lepton is represented by a four-component Dirac spinor $f^0_i$, where $i$ stands for the generation index and the superscript $0$ denotes interaction-eigenstates, and has two associated scalar superpartners, the sfermion $\tilde{f}^0_{Li}$ and the antisfermion $\tilde{f}^{0i\dagger}_R$, being related to the two-component holomorphic Weyl fermion $\chi_{fi}$ and antifermion $\chi_{\bar fi}$, respectively. Let us recall that we relate the Dirac fermion representations to the Weyl ones by
\be
   f_i^0 = \doublet{\chi_{fi}}{\bar\chi_{\bar fi}}.~
\ee For clarity, we will use in the following the left-handed component $f_{Li}^0$ and the right-handed component $f_{Ri}^0$ of the Dirac fermion $f_i^0$ and not the Weyl fermions $\chi_{fi}$ and $\chi_{\bar fi}$.
To preserve the electroweak symmetry from gauge anomaly and in order to give masses to both up-type and down-type fermions, the MSSM contains two Higgs doublets $H$, together with their fermionic partners, the higgsinos $\psi_{H}$,  
\be 
  H_u = \doublet{H_u^+}{H_u^0}, \qquad
  H_d = \doublet{H_d^0}{H_d^-}, \qquad
  \psi_{H_u} = \doublet{\psi_{H_u^+}}{\psi_{H_u^0}} {\rm ~~and~~}  
  \psi_{H_d} = \doublet{\psi_{H_d^0}}{\psi_{H_d^-}}.~
\ee 
Finally, the spin-one vector bosons of the Standard Model will be associated to Majorana fermions, the gauginos $\psi_B$, $\psi_{W^k}$ and $\psi_g$. 
The names and representations under the Standard Model gauge groups $SU(3)_C \times SU(2)_L \times U(1)_Y$ of the various fields are summarized in Table~\ref{tab:MSSMFieldContent}.\\



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent{\textbf{ Supersymmetry-conserving Lagrangian}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In order to have more compact notations, we introduce the $SU(2)_L$-doublets of left-handed fermions and sfermions,
\be
  Q^0_i = \doublet{u^0_{Li}}{d^0_{Li}} {\rm ~~,~~} 
  L^0_i = \doublet{\nu^0_i}{l^0_{Li}}  {\rm ~~,~~} 
  \tilde{Q}^0_i = \doublet{\tilde{u}^0_{Li}}{\tilde{d}^0_{Li}} {\rm ~~and~~} 
  \tilde{L}^0_i = \doublet{\tilde{\nu}^0_i}{\tilde{l}^0_{Li}},~
\ee the covariant derivative 
\be
  D_\mu = \del_\mu - i g_s T^a g_\mu^a - {1\over 2}i g \sigma^i W_\mu^i - i g^\prime Y B_\mu,~
\ee and the field strength tensors 
\be \bsp
  B_{\mu\nu}   =& \del_\mu B_\nu-\del_\nu B_\mu,\\
  W_{\mu\nu}^i =& \del_\mu W_\nu^i-\del_\nu W_\mu^i + g^\prime \,\epsilon^{ijk}\,W_\mu^j\,W_\nu^k,\\
  G_{\mu\nu}^a =& \del_\mu g_\nu^a-\del_\nu g_\mu^a + g_s\, f^{abc}\,g_\mu^b\,g_\nu^c.~
\esp\ee $g_s$, $g$ and $g'$ denote the three coupling constants associated with the $SU(3)_C\times SU(2)_L\times U(1)_Y$ gauge groups while $T$, $\sigma^i$ and $Y$ are the corresponding generators and $\epsilon^{ijk}$ represents the totally antisymmetric tensor. 



The pure gauge sector of the MSSM is identical as the Standard Model one. The Lagrangian is
\be
  \lag_{\rm Gauge} = 
    - {1\over 4}\,G_{\mu\nu}^a\,G^{\mu\nu}_a 
    - {1\over 4}\,W_{\mu\nu}^i\,W^{\mu\nu}_i
    - {1\over 4}\,B_{\mu\nu}\,B^{\mu\nu},~
\ee where we have not included any ghost term, since the present implementation of the model employs the unitary gauge. However, in order to have the CalcHEP model file computed by FeynRules to work, even in unitary gauge, we have to add the gluon ghost field $u_g^a$ in the Lagrangian,
\be 
  \lag_{\rm ghosts} = \bar u_g^a \del_\mu\, D^\mu u_{g,a}~
\ee The kinetic terms of the Lagrangian for quarks and leptons are also as in the Standard Model,
\be
  \lag_{\rm Fermions} = 
    \bar Q^{0i} i \slashed{D} \,Q^0_{i} + 
    \bar L^{0i}i \slashed{D}\, L^0_{i} + 
    \bar u^{0i}_R i\slashed{D} \,u^0_{Ri} +  
    \bar d^{0i}_R i\slashed{D} \,d^0_{Ri} +  
    \bar l^{0i}_R i\slashed{D}\,l^0_{Ri}.~
\ee 
The Lagrangian for the scalar sector can be divided into one purely kinetic part,
\be\bsp
  \lag_{\rm scalar \,\,kinetic} = &\, 
    D_\mu H_u^\dagger\, D^\mu H_u + 
    D_\mu H_d^\dagger\, D^\mu H_d + 
    D_\mu \tilde L^{0i \dagger}   \, D^\mu \tilde L^0_i + 
    D_\mu \tilde l_R^{0i \dagger} \, D^\mu \tilde l^0_{Ri}\\
  &\, + D_\mu \tilde Q^{0i \dagger}\,D^\mu \tilde Q^0_i +
    D_\mu \tilde u_R^{0i \dagger}\,D^\mu \tilde u^0_{Ri} + 
    D_\mu \tilde d_R^{0i \dagger}\,D^\mu \tilde d^0_{Ri},
\esp\ee and one part derived from the $D$-terms, the $F$-terms and the superpotential $W$. Indeed, auxiliary $F$- and $D$-fields must be added to the theory in order to preserve the supersymmetry when one goes off-shell, keeping the total number of fermionic and bosonic degrees of freedom equal. Solving their equations of motion leads, for a set of $n$ Dirac fermions $\{\psi_n\}$ and $2 n$ associated supersymmetric scalar partners $\{\phi_{Ln}, \phi^{n\dagger}_R\}$, to 
\be\bsp
  \lag_{\rm scalar \,\, FDW}=  &\, - W_L^i W_{Li}^\dagger -  W_R^i W_{Ri}^\dagger \\
  &\, - \frac{1}{2} \Big[ W^{ij}_{LL}\, \bar\psi_i^c P_L\psi_j + 2 W_{LR}^{ij}\, \bar\psi_i P_L\psi_j + W_{RR}^{ij}\, \bar\psi_i P_L\psi^c_j + \hc \Big]\\
  &\, - {1 \over 2} \Big[g\,(\phi_{L}^{i\dagger}T^a\phi_{Li}) - g\,(\phi^{i\dagger}_{R}T^a\phi_{Ri}) \Big] \Big[-g\,(\phi_{L}^{j\dagger}T^a\phi_{Lj}) +  g\,(\phi^{j\dagger}_{R}T^a\phi_{Rj}) \Big],~
\esp\ee where $\psi^c$ is the field charge-conjugated to $\psi$ and the derivates of the superpotential $W$ are given by 
\be \bsp
   W^i_L = & \frac{\del W}{\del\phi_{Li}} {\rm ~~and~~} W^i_R = \frac{\del W}{\del\phi_{Ri}}\\
   W^{ij}_{LL} = & \frac{\del^2 W}{\del\phi_{Li} \del\phi_{Lj}} {\rm ~~,~~} W^{ij}_{LR} = \frac{\del^2 W}{\del\phi_{Li} \del\phi_{Rj}} {\rm ~~and~~} W^{ij}_{RR} = \frac{\del^2 W}{\del\phi_{Ri} \del\phi_{Rj}}.~
\esp \ee Let us note that in the case of Majorana fermions, there is only one associated scalar field. In the framework of the MSSM, the superpotential reads 
\be \label{eq:superW}
   W_{MSSM} = 
     \tilde u_R^{0i\dagger}\,({\bf y^u})_i^{~j}\,(\tilde Q_j^0 \epsilon H_u) -
     \tilde d_R^{0i\dagger}\,({\bf y^d})_i^{~j}\,(\tilde Q_j^0 \epsilon H_d) - 
     \tilde l_R^{0i\dagger}\,({\bf y^l})_i^{~j}\,(\tilde L_j^0 \epsilon H_d) + 
     \mu \, H_u\epsilon H_d, 
\ee where ${\bf y^u}$, ${\bf y^d}$ and ${\bf y^l}$ denote the $3\times3$ Yukawa matrices, $\mu$ the Higgs off-diagonal mass-mixing, and $\epsilon$ the $SU(2)_L$ invariant tensor. We could add to this superpotential other gauge-invariant and renormalizable terms, but they would violate either the lepton number $L$ or the baryon number $B$, as well as the individual lepton flavours. Moreover, they allow for various $B$-violating or $L$-violating processes which have never been seen experimentally. We could in principle just  postulate $B$ and $L$ conservation, forbidding those terms, but however, neither $B$ nor $L$ are fundamental symmetries of nature since they are violated by non-perturbative electroweak effects \cite{'tHooft:1976up}. Therefore, an alternative symmetry is rather imposed, the $R$-parity \cite{Farrar:1978xj}, defined by 
\be 
   R =  (-1)^{3B+L+2S},~
\ee $S$ being the spin of the particle, forbidding any term different from those in Eq.\ (\ref{eq:superW}). All the Standard Model particles have thus a positive $R$-parity while the superpartners have a negative one. However, a $R$-parity violating extension of our implementation would be straightforward. We can now write the remaining part of the scalar Lagrangian, 
\be \bsp \label{eq:FDW}
  \lag_{\rm scalar \,\, FDW} = &\, -|\mu|^2\,\big(|H_u|^2+|H_d|^2\big)\\
  &\, + \bigg( \mu^\ast\, H_u^\dagger \Big[\tilde d_R^{0i\dagger}\,({\bf y^d})_i^{~j}\, \tilde Q_j^0 + \tilde l^{0i\dagger}_R\,({\bf y^l})_i^{~j}\,\tilde L_j^0 \Big]  
      + \mu^\ast\, H_d^\dagger \Big[\tilde u_R^{0i\dagger}\,({\bf y^u})_i^{~j}\, \tilde Q_j^0 \Big] +  \hc \bigg) \\  
  &\, + \big[H_u^\dagger\, \epsilon\, \tilde Q^{0i\dagger} \big] \, \big[{\bf y^u}^\dagger {\bf y^u} \big]_i^{~j} \, \big[\tilde Q_j^0\, \epsilon\, H_u\big]
      + \big[H_d^\dagger\, \epsilon\, \tilde Q^{0i\dagger} \big] \, \big[{\bf y^d}^\dagger {\bf y^d} \big]_i^{~j} \, \big[\tilde Q_j^0\, \epsilon\, H_d\big] \\
  &\, - \tilde u_R^{0i\dagger} \, \big[{\bf y^u}\, {\bf y^u}^\dagger\big]_i^{~j} \, \tilde u_{Rj}^0 \,\big|H_u\big|^2 
      - \tilde d_R^{0i\dagger} \, \big[{\bf y^d}\, {\bf y^d}^\dagger\big]_i^{~j} \, \tilde d_{Rj}^0 \,\big|H_d\big|^2\\
  &\, + \tilde u_R^{0i\dagger} \, \big[{\bf y^u}\, {\bf y^d}^\dagger\big]_i^{~j} \, \tilde d_{Rj}^0 \, H_d^\dagger H_u 
      + \tilde d_R^{0i\dagger} \, \big[{\bf y^d}\, {\bf y^u}^\dagger\big]_i^{~j} \, \tilde u_{Rj}^0\, H_u^\dagger H_d\\
  &\, + \big[H_d^\dagger\, \epsilon\, \tilde L^{0i\dagger} \big] \, \big[{\bf y^l}^\dagger {\bf y^l}\big]_i^{~j} \, \big[\tilde L^0_j\, \epsilon\, H_d\big] 
      - \tilde l_R^{0i\dagger} \, \big[{\bf y^l}\, {\bf y^l}^\dagger\big]_i^{~j} \, \tilde l_{Rj}^0\, \big|H_d\big|^2\\	
  &\, - \big[\tilde Q^{0j\dagger}\,({\bf y^u}^\dagger)_j^{~i}\,\tilde u_{Ri}^0\big] \, \big[\tilde u_R^{0k\dagger}\, ({\bf y^u})_k^{~l}\,\tilde Q_l^0\big] 
      - \big[\tilde Q^{0j\dagger}\,({\bf y^d}^\dagger)_j^{~i}\,\tilde d_{Ri}^0\big] \, \big[\tilde d_R^{0k\dagger}\, ({\bf y^d})_k^{~l}\,\tilde Q_l^0\big] \\
  &\, - \big[\tilde L^{0j\dagger}\,({\bf y^l}^\dagger)_j^{~i}\,\tilde l_{Ri}^0\big] \, \big[\tilde l_R^{0k\dagger}\, ({\bf y^l})_k^{~l}\,\tilde L_l^0\big] \\
  &\, - \big[\tilde Q^{0j\dagger}\,({\bf y^d}^\dagger)_j^{~i}\,\tilde d_{Ri}^0\big] \, \big[\tilde l_R^{0k\dagger}\,({\bf y^l})_k^{~l}\,\tilde L_l^0\big] 
      - \big[\tilde L^{0j\dagger}\,({\bf y^l}^\dagger)_j^{~i}\,\tilde l_{Ri}^0\big] \, \big[\tilde d_R^{0k\dagger}\,({\bf y^d})_k^{~l}\,\tilde Q_l^0\big] \\
  &\, -{1\over 2} \bigg[ 
         - {g^\prime \over 6} \, \tilde Q^{0i\dagger} \, \tilde Q_i^0 
	 + {g^\prime \over 2} \, \tilde L^{0i\dagger} \, \tilde L_i^0  
	 + {g^\prime \over 2} \, \tilde H_d^\dagger   \, \tilde H_d 
	 - {g^\prime \over 2} \, \tilde H_u^\dagger   \, \tilde H_u \\
  &\,\qquad 
         + {2 g^\prime \over 3}\, \tilde u_R^{0i\dagger} \, \tilde u_{Ri}^0 
	 - {g^\prime \over 3}  \, \tilde d_R^{0i\dagger} \, \tilde d_{Ri}^0 
	 - g^\prime            \, \tilde l_R^{0i\dagger} \, \tilde l_{Ri}^0 
     \bigg]^2 \\
  &\,-{1\over 2} \bigg[ 
         - {g \over 2} \, \tilde Q^{0i\dagger} \, \sigma^k \, \tilde Q_i^0 
	 - {g \over 2} \, \tilde L^{0i\dagger} \, \sigma^k \, \tilde L_i^0 
	 - {g \over 2} \, \tilde H_d^\dagger   \, \sigma^k \, \tilde H_d 
	 - {g \over 2} \, \tilde H_u^\dagger   \, \sigma^k \, \tilde H_u 
     \bigg]^2 \\
  &\, -{1\over 2} \bigg[
         - g_s \, \tilde Q^{0i\dagger}  \, T^a \, \tilde Q_i^0
	 + g_s \, \tilde u_R^{0i\dagger}\, T^a \, \tilde u_{Ri}^0
	 + g_s \, \tilde d_R^{0i\dagger}\, T^a \, \tilde d_{Ri}^0 
      \bigg]^2 .~
\esp\ee 
From the $W^{ij}$ terms of the superpotential, bilinear in the fermionic fields, we can also generate the Yukawa couplings between the matter fermions and the Higgs fields,  
\be
  \lag_{\rm Yukawa} = - \bar u_R^{0i} ({\bf y^u})^{~j}_i  \, Q_j^0 \, \epsilon \, H_u
    + \bar d_R^{0i} ({\bf y^d})^{~j}_i  \, Q_j^0 \, \epsilon \, H_d
    + \bar l_R^{0i} ({\bf y^l})^{~j}_i  \, L_j^0 \, \epsilon \, H_d
    + \hc ~
\ee
The terms of the MSSM Lagrangian containing higgsino and gaugino fields can be divided into three parts; pure kinetic terms, 
\be
  \lag_{\rm ino\,\, kinetic} = 
    {1 \over 2} \bar \psi_B    \, i \slashed{\del} \, \psi_B + 
    {1 \over 2} \bar \psi_{W^k}\, i \slashed{D}    \, \psi_{W^k} + 
    {1 \over 2} \bar \psi_{g^a}\, i \slashed{D}    \, \psi_{g^a} + 
    {1 \over 2} \bar \psi_{H_u}\, i \slashed{D}    \, \psi_{H_u} + 
    {1 \over 2} \bar \psi_{H_d}\, i \slashed{D}    \, \psi_{H_d},~
\ee Yukawa interactions obtained from the superpotential terms $W_{ij}$, 
\be\bsp
   \lag_{\rm ino\, \, Yukawa} =&\, 
     - \big[\bar u_R^{0i}\,  \epsilon\,\psi_{H_u} \big]\, ({\bf y^u})_i^{~j}\, \tilde Q^0_j \,
     + \big[\bar d_R^{0i}\,  \epsilon\,\psi_{H_d} \big]\, ({\bf y^d})_i^{~j}\, \tilde Q^0_j \,
     + \big[\bar l_R^{0i}\,  \epsilon\,\psi_{H_d} \big]\, ({\bf y^l})_i^{~j}\, \tilde L^0_j\\
   &\, - \tilde u_R^{0i\dagger}\, ({\bf y^u})_i^{~j}\, \big[ \bar Q_j^{c\,0}\, \epsilon\, \psi_{H_u} \big] \, 
       + \tilde d_R^{0i\dagger}\, ({\bf y^d})_i^{~j}\, \big[ \bar Q_j^{c\,0}\, \epsilon\, \psi_{H_d} \big] \, 
       + \tilde l_R^{0i\dagger}\, ({\bf y^l})_i^{~j}\, \big[ \bar L_j^{c\,0}\, \epsilon\, \psi_{H_d} \big]\\
   &\, - {1 \over 2} \mu\, \big( \bar \psi_{H_u} \, \epsilon\,  P_L \,\psi_{H_d} + \bar \psi_{H_d} \, \epsilon\, P_L \, \psi_{H_u} \big) + \hc~,~
\esp\ee and additional supersymmetry-conserving gauge-like interactions which have no counterpart in the Standard Model and which are not taken into account through the covariant derivatives, 
\be\bsp
  \lag_{\rm ino\, \, mix} =
    &\, \sqrt{2} g^\prime \Big[ - {1 \over 6} \tilde Q^{0i\dagger}\, \big(\bar Q_i^{c\,0}\, \psi_{B}\big) 
                                + {1 \over 2} \tilde L^{0i\dagger}\, \big(\bar L_i^{c\,0}\, \psi_{B}\big) \Big] + \hc \\
    &\, \sqrt{2} g^\prime \Big[   {2 \over 3} \big(\bar\psi_{B}\, u_R^{0i}\big)\, \tilde u_{Ri}^0
		   	        - {1 \over 3} \big(\bar\psi_{B}\, d_R^{0i}\big)\, \tilde d_{Ri}^0 
			        - \big(\bar\psi_{B}\,l_R^{0i}\big)\, \tilde l_{Ri}^0 \Big] + \hc \\
    &\,- {g \over \sqrt{2}} \Big[   \tilde Q^{0i\dagger}\, \sigma^k\, \big(\bar Q_i^{c\,0}\, \psi_{W^k}\big) 
                                  + \tilde L^{0i\dagger}\, \sigma^k\, \big(\bar L_i^{c\,0}\, \psi_{W^k}\big) \Big] + \hc\\
    &\,+ \sqrt{2} g_s \Big[ - \tilde Q^{0i\dagger}\, T^a\, \big(\bar Q_i^{c\,0}\, \psi_{g^a}\big) 
                            + \big(\bar\psi_{g^a}\, u_R^{0i}\big)\, T^a\, \tilde u_{Ri}^0 
			    + \big(\bar\psi_{g^a}\, d_R^{0i}\big)\, T^a\, \tilde d_{Ri}^0 \Big] + \hc~
\esp\ee


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent{\textbf{ Supersymmetry-breaking Lagrangian}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

As stated in the introduction, the masses of the superpartners must be considerably larger than those of the Standard Model particles. Realistic supersymmetric models must hence include supersymmetry breaking, which is expected to occur spontaneously. The Lagrangian density will then respect supersymmetry invariance, but the vacuum state does not. Moreover, in order not to introduce quadratic divergences in loop-calculations, the breaking has to be soft. In practice, since we do not know the supersymmetry-breaking mechanism and the corresponding scale, we will add all possible terms breaking explicitly the supersymmetry at low-energy \cite{Girardello:1981wz},
\be \bsp \label{eq:lsoft}
   \lag_{\rm soft} =
   &\,- {1 \over 2} \Big[ M_1 \bar\psi_{B}\, \psi_{B} + M_2\,\bar \psi_{W^k}\, \psi_{W^k} + M_3\,\bar \psi_{g^a}\, \psi_{g^a} \Big]\\
   &\,- \,\tilde Q^{0i\dagger}\,({\bf m^2_{\tilde Q}})_i^{~j}\,\tilde Q^0_j - \,\tilde u_R^{0i\dagger}\,({\bf m^2_{\tilde U}})_i^{~j}\,\tilde u_{Rj}^0 - \,\tilde d_R^{0i\dagger}\,({\bf m^2_{\tilde D}})_i^{~j}\,\tilde d_{Rj}^0 \\
   &\,- \,\tilde L^{0i\dagger}  \, ({\bf m^2_{\tilde L}})_i^{~j}\, \tilde L^0_j - \,\tilde l_R^{0i\dagger}\, ({\bf m^2_{\tilde E}})_i^{~j}\, \tilde l_{Rj}^0 \\ 
   &\,- \, m_{H_u}^2\, H_u^\dagger\, \epsilon\, H_u  - \, m_{H_d}^2\, H_d^\dagger\, \epsilon\, H_d  - \, b\,      H_u\,         \epsilon\, H_d\,  - \, b^\ast\, H_u^\dagger\, \epsilon\, H_d^\dagger\\
   &\,+ \Big[ -\,\tilde u_R^{0i\dagger}\, ({\bf a_u})_i^{~j}\, \tilde Q_j^0\, \epsilon H_u 
              +\,\tilde d_R^{0i\dagger}\, ({\bf a_d})_i^{~j}\, \tilde Q_j^0\, \epsilon H_d 
	      +\,\tilde l_R^{0i\dagger}\, ({\bf a_l})_i^{~j}\, \tilde L_j^0\, \epsilon H_d \,\,+\, \hc \Big].
\esp \ee
The first line of Eq.\ (\ref{eq:lsoft}) contains gaugino mass terms, the second and third lines the sfermion mass terms, where ${\bf m^2_{\tilde Q}}$, ${\bf m^2_{\tilde L}}$, ${\bf m^2_{\tilde u}}$, ${\bf m^2_{\tilde d}}$, ${\bf m^2_{\tilde e}}$ are $3\times3$ hermitian matrices in generation space, the fourth line mass terms for the Higgs fields, and the fifth line the trilinear scalar interactions, ${\bf a_u}$, ${\bf a_d}$, and ${\bf a_e}$ being also $3\times 3$ matrices in generation space. Note that the additional Higgs mass terms are required in order to break electroweak symmetry spontaneously.\\ 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent{\textbf{Full Lagrangian}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We finally obtain the full MSSM Lagrangian
\be \bsp
\lag_{\rm susy} = 
  &\, \lag_{\rm Fermions} + \lag_{\rm Gauge} + \lag_{\rm scalar \,\,kinetic} + \lag_{\rm scalar \,\, FDW} + \lag_{\rm Yukawa}\\ 
  &\, + \lag_{\rm ino\,\, kinetic} + \lag_{\rm ino\, \, Yukawa} + \lag_{\rm ino\, \, mix} + \lag_{\rm soft}
\esp \ee collecting the various pieces given above. So far, everything is expressed in terms of interaction-eigenstates. However, non-diagonal mass matrices arise after electroweak symmetry breaking and they need to be diagonalized. This issue will be addressed in the next section.\\



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent{\textbf{Particle mixing}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In order to break the electroweak symmetry to electromagnetism, the classical Higgs potential, \ie \! all the Lagrangian terms quadratic or quartic in the Higgs fields, must have a non-trivial minimum. Due to gauge invariance, one of the charged Higgs vacuum expectation value (vev) can be rotated away, which yields a zero vev for the other charged Higgs. Again, we can use gauge-invariance to choose the remaining vevs real and positive, so that we can replace the neutral Higgs fields in $\lag_{\rm susy}$ by
\be
  H_u^0 \to  {v_u + h_u^0 \over \sqrt{2}} {\rm ~~and~~} 
  H_d^0 \to  {v_d + h_d^0 \over \sqrt{2}},~
\ee where $v_u$ and $v_d$ are the two vacuum expectation values of the neutral Higgses and $h_u^0$ and $h_d^0$ are complex scalar fields. Let us note that those relations are only valid in unitary gauge, which is the case we are dealing with. We can then extract mass matrices for the gauge bosons $B^0$ and $W^k$, diagonalize them, and derive the physical mass-eigenstates, the photon $A$, the $W$- and $Z$-boson. The transformation rules relating the mass and interaction bases are given by
\ba \label{eq:Wmixing}
   W^1_\mu =\,\, {1 \over \sqrt{2}} \big( W^-_\mu + W^+_\mu \big) &{\rm~~and~~}&
   W^2_\mu =\,\, {1 \over \sqrt{2} i} \big( W^-_\mu - W^+_\mu \big), ~\\
   W^3_\mu =\,\,  \cw\, Z_\mu + \sw\, A_\mu &{\rm~~and~~}&
   B^0_\mu =\,\, -\sw\, Z_\mu + \cw\, A_\mu .~
\ea  The weak mixing angle $\theta_w$ and the physical masses $m_Z$ and $m_W$ are defined by
\be
   \cwd = {g^2 \over g^2+g^{\prime 2}}{~~,~~}
   m_Z^2 = {g \over 2 \cw} \sqrt{v_u^2+v_d^2} {\rm ~~and~~}
   m_W^2 = {g \over 2} \sqrt{v_u^2+v_d^2}.~
\ee
In the Higgs sector, three out of the eight real degrees of freedom of the two doublets are the would-be Nambu-Goldstone bosons becoming the longitudinal modes of the weak bosons, while the five others mix to the physical Higgses, $h^0$, $H^0$, $A^0$ and $H^\pm$. The diagonalization of several mass matrices yields to the transformation rules
\ba
  h_u^0 =  \ca\, h^0 + \sa\, H^0 + i \cb\, A^0 &{\rm~~and~~}& h_d^0 = -\sa\, h^0 + \ca\, H^0 + i \sb\, A^0 , ~~~~~~~~\\ 
  H_u^+ =  \cb\, H^+ &{\rm~~and~~}& H_d^- = \sb\, H^-,~
\ea where $\tb$ is the ratio of the two vevs $v_u$ and $v_d$.



 
Collecting the terms of $\lag_{\rm susy}$ bilinear in the Majorana fermions $\psi_{B}$, $\psi_{W^3}$, $\psi_{H_u^0}$ and $\psi_{H_d^0}$, we can extract the neutral gaugino-higgsino mass matrix $Y$ which can be diagonalized through a unitary matrix $N$,
\be
 N^\ast\, Y\, N^{-1} ={\rm diag}\, (m_{\tilde{\chi}^0_1},m_{\tilde{\chi}^0_2},
 m_{\tilde{\chi}^0_3},m_{\tilde{\chi}^0_4}).~
\ee This matrix relates the four physical neutralinos $\tilde \chi^0_i$ to the interaction-eigenstates,
\be 
  (\tilde{\chi}^0_1\,\,\, \tilde{\chi}^0_2\,\,\,  \tilde{\chi}^0_3\,\,\, \tilde{\chi}^0_4)^T = N \, (\psi_{B}\,\,\,  \psi_{W^3}\,\,\,  \psi_{H_d^0}\,\,\,  \psi_{H_u^0})^T.~
\ee Similarly, we can collect the terms yielding the charged gaugino-higgsino mass matrix $X$ and diagonalize it through the two unitary matrices $U$ and $V$,
\be
 U^\ast\, X\, V^{-1} = {\rm diag}\,(m_{\tilde{\chi}^\pm_1},m_{\tilde{\chi}^ \pm_2}).~
\ee Those matrices relate the interaction-eigenstates to the physical charginos $\tilde \chi^\pm_i$
\be
  (\tilde{\chi}^+_1\,\,\, \tilde{\chi}^+_2)^T = V (\psi_{W^+}\, \, \, \psi_{H^+_u})^T {\rm~~and~~}  (\tilde{\chi}^-_1\,\,\, \tilde{\chi}^-_2)^T = U (\psi_{W^-}\, \,\, \psi_{H^-_d})^T.~
\ee
Note that the fields $\psi_{W^\pm}$ are obtained after rotating $\psi_{W^1}$ and $\psi_{W^2}$ as in Eq.\ (\ref{eq:Wmixing}) for the $W$-boson.



Within the Standard Model, the only source of flavour violation arises through the rotation of the up-type and down-type quark interaction-eigenstates basis $\{d_{Li}^0,u_{Li}^0,d_{Ri}^0,u_{Ri}^0\}$ to the basis of the physical mass eigenstates $\{d_{Li},u_{Li},d_{Ri},u_{Ri}\}$ in which the Yukawa matrices ${\bf y^u}$ and ${\bf y^d}$ are diagonal. This diagonalization requires four unitary matrices 
\be
  d_{Li}^0 = V_d\, d_{Li}\,, \quad d_{Ri}^0 = U_d\, d_R\,, \quad  u_{Li}^0 = V_u\, u_{Li}\,, \quad u_{Ri}^0 = U_u\, u_R\,, 
\ee and render the charged-current interactions proportional to the CKM matrix \cite{Cabibbo:1963yz, Kobayashi:1973fv}, 
\be
  V_{\rm CKM}=V_u^\dagger V_d~.~
\ee The leptonic sector is however diagonalized with the help of only two matrices, since the neutrinos are assumed massless,
\be
  l_{Li}^0 = V_l\, l_{Li}\,, \quad l_{Ri}^0 = U_l\, l_R\,, \quad 
  \nu_i^0 = \nu_i\,.~
\ee Note that the matrices $U_u$, $U_d$, $V_l$ and $U_l$ do not appear in the rotated Lagrangian. 
In the sfermion sector, we define the super-CKM basis  \cite{Hall:1985dx} as the basis in which the sfermion interaction-eigenstates undergo the same rotations as their fermionic counterparts. As a consequence, the squark charged-current interactions are also proportional to the CKM matrix. However, the fermion and sfermion fields can be misaligned due to possible off-diagonal mass terms in the supersymmetry-breaking Lagrangian $\lag_{\rm soft}$. The diagonalization of the four mass matrices $M_{\tilde{u}}^2$, $M_{\tilde{d}}^2$, $M_{\tilde{l}}^2$ and $M_{\tilde{\nu}}^2$ requires thus the introduction of three $6 \times 6$ matrices $R^u$, $R^d$ and $R^l$ and one $3 \times 3$ matrix $R^\nu$,
\ba
  {\rm diag}\,(m_{\tilde u_1}^2, \ldots, m_{\tilde u_6}^2) ~=~ R^u\, M_{\tilde{u}}^2\,R^{u\dag} &{\rm ~~~~,~~~~}& {\rm diag}\,(m_{\tilde d_1}^2, \ldots, m_{\tilde d_6}^2) ~=~ R^d\, M_{\tilde{d}}^2\, R^{d\dag},\\
  {\rm diag}\,(m_{\tilde \nu_1}^2, \ldots, m_{\tilde \nu_3}^2) ~=~ R^\nu\, M_{\tilde{\nu}}^2\,R^{\nu\dag} &{\rm ~~~~,~~~~}& {\rm diag}\,(m_{\tilde l_1}^2, \ldots, m_{\tilde l_6}^2) ~=~ R^l\, M_{\tilde{l}}^2\, R^{l\dag},~
\ea These matrices relate the physical mass-eigenstates to the interaction-eigenstates through 
\be \bsp
  (\tilde{u}_1, \tilde{u}_2, \tilde{u}_3, \tilde{u}_4, \tilde{u}_5, \tilde{u}_6)^T =& R^u\, (\tilde{u}_L, \tilde{c}_L, \tilde{t}_L, \tilde{u}_R, \tilde{c}_R, \tilde{t}_R)^T ,\\
  (\tilde{d}_1, \tilde{d}_2, \tilde{d}_3, \tilde{d}_4, \tilde{d}_5, \tilde{d}_6)^T =& R^d\, (\tilde{d}_L, \tilde{s}_L, \tilde{b}_L, \tilde{d}_R, \tilde{s}_R, \tilde{b}_R)^T , \\
  (\tilde{\nu}_1, \tilde{\nu}_2, \tilde{\nu}_3)^T =& R^\nu\, (\tilde{\nu}_e, \tilde{\nu}_\mu, \tilde{\nu}_\tau)^T,~\\
  (\tilde{l}_1, \tilde{l}_2, \tilde{l}_3, \tilde{l}_4, \tilde{l}_5,  \tilde{l}_6)^T =& R^l\, (\tilde{e}_L, \tilde{\mu}_L, \tilde{\tau}_L, \tilde{e}_R, \tilde{\mu}_R, \tilde{\tau}_R)^T.~ 
\esp\ee
The less general built-in implementation of the MSSM in MadGraph and CalcHEP can easily be recovered by setting all the off-diagonal elements of these general mixing matrices to zero, except for the third generation flavour-conserving and helicity-mixing elements.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Checks and validation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent{\textbf{Analytical checks}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In order to validate our implementation, we have first compared the Feynman Rules computed by FeynRules to those which can be found in the litterature, both for the general MSSM \cite{Rosiek:1989rs, Rosiek:1995kg} and for a simplified MSSM where all the scalar mixings are neglected \cite{Haber:1984rc, Gunion:1984yn}. We have a full agreement for all the vertices. 
Then, using the FeynArts/FormCalc interface, we have produced a model file for the most general MSSM. Using the two programs, we have re-calculated all squark and gaugino hadroproduction helicity amplitudes in the case of general (and possibly complex) scalar mixing. The results have been compared to the analytical formulas given in Refs.\ \cite{Bozzi:2007me, Fuks:2008ab} and we obtain a complete agreement.\\


 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent{\textbf{Strategy for the validation of the Monte-Carlo generator model files}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Presently, we have only validated the model files produced for MadGraph and CalcHEP. However, extensions of the validation process to the SHERPA generator or to any other program which will be interfaced to FeynRules in the future are possible and even planned for SHERPA. The built-in implementations of the MSSM in MadGraph/MadEvent and CalcHEP hold in the very particular limit where CP symmetry and flavour are assumed to be conserved within the whole model, the CKM matrix appearing in the charged-current interactions being thus neglected as well. In addition, in the scalar sector, the flavour-conserving helicity mixings are neglected for first and second generation sfermions. Apart from these simplifications which we can easily handle with our general implementation of the MSSM, \ie \! fixing the relevant parameters to zero or one, we still need to assume a supersymmetry-breaking scenario. We choose the typical minimal supergravity point SPS 1a \cite{Allanach:2002nj} which is completely defined once we fix the values of four parameters at the gauge coupling unification scale and one sign,
\be
  m_0=100 {\rm~GeV~}, \quad m_{1/2}=250 {\rm~GeV~}, \quad A_0=-100 {\rm~GeV~}, \quad \tb=10, \quad {\rm~~and~~} \mu>0.~
\ee $m_0$ and $m_{1/2}$ are the universal scalar and gaugino masses, $A_0$ is the universal trilinear coupling, and as in the previous section, $\tb$ is the ratio of the two vacuum expectation values of the Higgs fields and $\mu$ is the off-diagonal Higgs mixing parameter. We use the numerical program SOFTSUSY \cite{Allanach:2001kg} to solve the renormalization group equations linking this restricted set of supersymmetry-breaking parameters at high-energy scale to the complete set of masses, mixing matrices and parameters appearing in $\lag_{\rm susy}$ at the weak scale. The complete list of the values for those parameters is encoded in a file following the SLHA conventions, readable by FeynRules after the use of an additional translation interface in order to take into account the small differences between the SLHA format and the one of our implementation. This interface is available on the FeynRules website.



Starting from our general implementation of the MSSM, we first read the input parameters and use the FeynRules interfaces to implement the model files for the two matrix-element generators MadGraph and CalcHEP. In the following, we will denote those model files MG-FR and CH-FR, respectively, whereas the built-in (stock) implementations will be denoted MG-ST and CH-ST. Let us remark that since CalcHEP is not able to deal with files following the SLHA conventions, we had to modify the built-in files in order to correctly fix the free parameters of the model, while MadGraph was directly able to read the SLHA file produced by SOFTSUSY and use the provided values.\\



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent{\textbf{Decay widths}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We start by evaluating the 320 kinematically allowed two-body decay widths of supersymmetric and Standard Model particles in order to check the norm of various three-point vertices. We find a complete agreement both for processes from the Standard Model sector
\be 
  t      \to b   \, W,                 \quad  
  V      \to f   \, \bar f^{(\prime)}, \quad 
  \phi   \to f   \, \bar f^{(\prime)}, \quad  
  H^0    \to h^0 \, h^0,~
\ee and for processes from the supersymmetric sector,
\be
  \tilde f_i    \to \tilde \chi_j        \, f^\prime, \quad
  \tilde f_i    \to \tilde f_j^\prime    \, V,        \quad
  \tilde f_i    \to \tilde f_j^\prime    \, \phi,     \quad
  \tilde g      \to \tilde f_j           \, f^\prime, \quad
  \tilde \chi_i \to \tilde f_j           \, f^\prime, \quad
  \tilde \chi_i \to \tilde \chi_j^\prime \, V,        \quad
  \tilde \chi_i \to \tilde \chi_j^\prime \, \phi,     \quad
\ee $f^{(\prime)}$ being any Standard Model fermion, $V$ any gauge boson, $\phi$ any Higgs field, $\tilde f_i^{(\prime)}$  any sfermion and $\tilde \chi_j$ any chargino or neutralino. For those checks, we have confronted the MG-FR implementation to the already validated MG-ST implementation \cite{Hagiwara:2005wg}, and the agreement between the two predictions was evaluated through the quantity
\be \label{eq:delta}
   \Delta = 2\,  {\big| \Gamma^{FR} - \Gamma^{ST}\big| \over \Gamma^{FR} + \Gamma^{ST}},~
\ee For all the channels, $\Delta$ has been found to be smaller than one percent, the remaining differences being hence associated to a pure Monte-Carlo uncertainty. The results for the most important kinematically allowed decay channels can be found in Appendix \ref{App:SUSYTablesDecay}. For consistency, we have also tested the charge-conjugate decays.\\



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent{\textbf{$2\to 2$ processes}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


The second stage in the validation of the model files computed by FeynRules consists in the evaluation of the total cross section for several $2\to 2$ processes, and this with the help of both MadGraph and CalcHEP. We will at the same time confront our results to those obtained with both built-in implementations of the MSSM. We have checked that the six quantities  $\Delta_{ab}$ generalizing Eq.\ (\ref{eq:delta}) for any set of two predictions $a$ and $b$,
\be \label{eq:deltaPS}
   \Delta_{ab} = 2\,  {\big| \sigma^a - \sigma^b\big| \over \sigma^a + \sigma^b},~
\ee are below the percent level. Regarding the two MadGraph model files alone, this check allows not only to verify the correctness of all the three-point vertices and some four-point ones, but also to start being sensitive to the global sign of a large part of those vertices, since for most of the processes that we have evaluted, there are several interfering Feynman diagrams contrary to the two-body decays depending only on a single diagram. This is also the first comparison between predictions obtained with MadGraph and with CalcHEP for the MSSM, which would be an important check since CalcHEP and MadGraph have never been confronted into the past, at least for the MSSM. We have considered the production of either a pair of any Standard Model particles, or a pair of any supersymmetric particles, and the initial states
\be\bsp
 & e^+    \, e^-           ,\quad 
  \tau^+ \, \tau^-        ,\quad
  e^-    \, \bar \nu_e    ,\quad
  e^-    \, e^-           ,\quad
  \tau^- \, \bar \nu_\tau ,\quad \\&
  u      \, \bar u        ,\quad
  d      \, \bar d        ,\quad
  b      \, \bar b        ,\quad
  b      \, \bar t        ,\quad
  u      \, u             ,\quad
  d      \, d             ,\quad
  u      \, g             ,\quad
  d      \, g             ,\quad \\&
  W^+    \, W^-           ,\quad
  W^-    \, Z             ,\quad
  W^-    \, \gamma        ,\quad
  Z      \, Z             ,\quad
  Z      \, \gamma        ,\quad
  \gamma \, \gamma        ,\quad
  g      \, \gamma        ,\quad
  g      \, Z             ,\quad
  g      \, W^\pm         ,\quad
  g      \, g             .~
\esp \ee The key in evaluating those not really phenomenologically relevant channels, since most of the initial state are impossible to realize at a collider, is to really allow us to be sensitive to \textit{each} three-point vertex embedded in the Lagrangian, and a large part of the four-point vertices. Let us note that the remaining untested vertices, such as the four-scalar interactions in $\lag_{\rm scalar\, \, FDW}$ in Eq.\ (\ref{eq:FDW}), are irrelevant for $2\to 2$ leading-order calculations with a Standard Model initial state. We have considered two different cases, one where we have fixed the  energies of the initial particles to 600 GeV, and one to 1 TeV. In total, we have investigated 456 different channels.



From the predictions for the production of a pair of any Standard Model particles, we can calculate the six $\Delta_{ab}$ quantities and verify that the four implementations, MG-FR, MG-ST, CH-FR, CH-ST are in agreement below the percent level. The results for the processes yielding the largest cross sections can be found in Appendix \ref{App:SUSYTables2to2SM}. Let us recall that the complete list is available on the FeynRules webpage. We found a complete agreement for most of the processes, except for 
\be\bsp
&e^+    \, e^-           \to V \, V,    ~~
\tau^+ \, \tau^-        \to Z   \, Z,      ~~
e^-    \, \bar \nu_e    \to Z   \, W^-,    ~~
\tau^- \, \bar \nu_\tau \to Z   \, W^-,    ~~
\tau^+ \, \tau^-        \to V \, V,    \\
&u      \, \bar u        \to V \, V,    ~~
u      \, \bar u        \to Z   \, Z,      ~~
d      \, \bar d        \to V \, V,    ~~
d      \, \bar d        \to Z   \, Z,      ~~
b      \, \bar t        \to Z   \, W^-,    \\
&W^+    \, W^-           \to V \, V,    ~~
g      \, g             \to t   \, \bar t,~
\esp \ee with two 600 GeV initial particles and for 
\be\bsp
& e^+    \, e^-          \to Z   \, Z,   ~~
\tau^+ \, \tau^-        \to Z   \, Z,   \\
& W^+    \, W^-           \to W^+ \, W^-,  ~~
Z      \, \gamma        \to W^+ \, W^-,\\
& u      \, \bar u        \to Z   \, Z,   ~~
d      \, \bar d        \to Z   \, Z,~
\esp \ee with two 1000 GeV beams. $V$ denotes either a $Z$- or a $W$-boson. Even if we have a complete agreement regarding the two implementations in CalcHEP, some discrepancies are due to the presence of $t$-channel diagrams with massless propagator, leading to numerical instabilities once we are running MadGraph. In order to avoid those instabilities and confront the two MadGraph implementations, we have calculated the squared matrix elements $|M^{FR}|^2$ and $|M^{ST}|^2$ at given phase space points for both models and computed the quantity
\be
\Delta^{PS} = \sum_{\rm phase\,\, space\,\, points} \Bigg\{2\,  {\Big| |M^{FR}|^2 - |M^{ST}|^2\Big| \over |M^{FR}|^2 + |M^{ST}|^2} \Bigg\}.~
\ee For 100 different random phase space points, we have found that $\Delta^{PS}$ is smaller than $0.1\%$ for all the problematic processes, as it is shown in Appendix \ref{App:SUSYTables2to2SM}, which validate the MG-FR implementations versus MadGraph the built-in one. 



We now turn to the production of a pair of supersymmetric particles from a fermionic initial state. For almost all the considered processes, we found that all the $\Delta_{ab}$ quantities are below the percent level. However, we have identified two classes of processes where at least one of the implementation does not agree with the others. For the processes
\be
  \tau^+ \, \tau^- \to \tilde l_1^+ \, \tilde l_6^-, \quad 
  b \, \bar b \to \tilde u_6 \, \tilde u_6^\dagger, \quad 
  b \, \bar b \to \tilde u_1 \, \tilde u_6^\dagger \quad {\rm and} \quad 
  b \, \bar b \to \tilde \chi_1^0 \, \tilde \chi_1^0,~
\ee the CH-ST implementation gives wrong results due to mistakes in several triple scalar couplings, and this either with two initial beams of 600 GeV, or of 1000 GeV, regarding the relative size of the different diagrams at the two energies. For 
\be \bsp
&  e^+ \, e^- \to \tilde l_5^- \, \tilde l_2^+, \quad  
  \tau^+ \, \tau^- \to h^0\,  h^0, \quad
  \tau^+ \, \tau^- \to h^0\,  H^0, \quad
  \tau^+ \, \tau^- \to h^0\,  A^0, \\
&  \tau^+ \, \bar \nu_\tau \to H^- \, h^0 \quad  {\rm and} \quad
  b \, \bar b \to h^0\,  h^0,~
\esp \ee
MadGraph disagrees with CalcHEP for one of the two possible initial energies. In most of the case, we have even a disagreement between the two MadGraph implementations as well. However, we have found a complete agreement after comparing matrix element calculations at given random phase space points. We can thus conclude that the discrepancies are coming from numerical instabilities in the way MadGraph is performing the cross section calculations. Some numerical examples are shown in Appendices \ref{App:SUSYTables2to2SUSYee} and \ref{App:SUSYTables2to2SUSYqq}.


Considering two gauge bosons in the initial state, we have computed the $\Delta_{ab}$ quantities for the production of any pair of supersymmetric particles and we have found them below the percent level, except for the processes
\be\bsp
& V   \, V \to \tilde l_1^- \, \tilde l_1^+         \quad
V   \, V \to \tilde l_6^- \, \tilde l_6^+         \quad
V   \, V \to \tilde l_1^- \, \tilde l_6^+         \\&
V   \, V \to \tilde u_1   \, \tilde u_1^\dagger,  \quad
V   \, V \to \tilde u_4   \, \tilde u_4^\dagger,  \quad
V   \, V \to \tilde u_5   \, \tilde u_5^\dagger,  \quad
V   \, V \to \tilde u_6   \, \tilde u_6^\dagger,  \quad
V   \, V \to \tilde u_1   \, \tilde u_6^\dagger,  \\&
V   \, V \to \tilde d_1   \, \tilde d_1^\dagger,  \quad
V   \, V \to \tilde d_2   \, \tilde d_2^\dagger,  \quad
V   \, V \to \tilde d_5   \, \tilde d_5^\dagger,  \quad
V   \, V \to \tilde d_6   \, \tilde d_6^\dagger,  \quad
V   \, V \to \tilde d_1   \, \tilde d_2^\dagger,  \\&
V   \, V \to h^0          \, h^0,                 \quad
V   \, V \to h^0          \, H^0,                 \\&
W^- \, Z \to \tilde d_2 \, \tilde u_1^\dagger,    \\&
g   \, g \to \tilde q_i   \, \tilde q_j^\dagger.~
\esp \ee where $VV$ stands for $W^+ W^-$ or $ZZ$. Again, we have here the two different classes of problems mentionned above, several bugs in the built-in implementation of the MSSM in CalcHEP, together with a different treatment of the cancellation between destructively interfering diagrams in MadGraph and CalcHEP yielding to discrepancies. This holds both for 600 GeV and 1000 GeV beams in the initial state, except for the production of a pair of squarks which is source of problems only for 600 GeV beams. A summary of the results can be found in Appendix \ref{App:SUSYTables2to2SUSYVV}.

Finally, we have compared the results for quark-gluon initiated processes and fermion-pair scattering (contrary to a fermion-antifermion initial state). We have agreement for all processes but
\be
e^- \, e^- \to \tilde l_5^- \, \tilde l_5^- \quad {\rm and} \quad 
e^- \, e^- \to \tilde l_2^-\, \tilde l_2^-,~
\ee for 600 GeV beams where the two MadGraph implementations disagree with the two CalcHEP ones. In one case, MG-FR and MG-ST give the same results, while in the other they do not. We have compared squared matrix elements for the two MadGraph implementations, and they are equal, from which we can again conclude to a numerical issue in MadGraph. Some cross sections are given in Appendix \ref{App:SUSYTables2to2SUSYother}.\\



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent{\textbf{$2\to 3$ processes}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Finally, in order to test \textit{every} sign of each three-point vertex and a large part of the four-point vertices (even some of the four-scalar ones), we have evaluated squared matrix elements for 100 random phase space points and calculated the quantity $\Delta^{PS}$ defined in Eq.\ (\ref{eq:deltaPS}). We have investigated 2708 processes, relative to the production of two supersymmetric particle plus one Standard Model particle at a center-of-mass energy of 2000 GeV. Using MG-FR and MG-ST, we have found a complete agreement for each process, i.e.\ $\Delta^{PS}$ was below 0.1 $\%$. A selection of the results is given in Appendix \ref{App:SUSYTables2to3}. The comparison with matrix element calculated with CH-FR and CH-ST is devoted to a further study.




\subsection{3-site and Moose Models (Neil)}
\subsection{Extra Dimensional models (Priscila)}
\subsection{Effective lagrangians : Non-linear sigma model and SILH models (Celine, Swarup)}
\subsection{Exotic models : the non-commutative SM, Hidden Valley Models (Claude)}

\section{Outlook (Fabio)}

\acknowledgments{We are indebted with many people and especially to Semenov who, by refusing to have
LanHEP interfaced to MadGraph three years ago, spurred us to engage in this project.
This work was partially supported by the Institut Interuniversitaire des Sciences Nucl\'eaires and by the Belgian Federal Office for Scientific, Technical and Cultural Affairs through the Interuniversity Attraction Pole P6/11. It is also part of the research program of the ``Stichting voor Fundamenteel Onderzoek der Materie (FOM)", which is financially supported by the ``Nederlandse organisatie voor Wetenschappelijke Onderzoek (NWO)".}

\appendix

\section{Interfaces (Fabio)}
\subsection{CalcHEP (Neil)}
\subsection{FeynArts/FormCalc (Benjamin or Claude}
\subsection{MadGraph/MadEvent (Michel)}
\subsection{SHERPA (Steffen)}

\vskip1cm
\section{Validation tables}
\subsection{The most general 2HDM (Michel)}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{The most general MSSM}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We list here some of the decay widths and cross sections which we have calculated in order to validate the model files for MadGraph and CalcHEP computed by FeynRules. These implementations are denoted by MG-FR and CH-FR, respectively, and we recall that the built-in implementations are denoted by MG-ST and CH-ST. A more complete list of results of the checks can be found on the FeynRules webpage.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{\textbf{Decay widths}}
\label{App:SUSYTablesDecay}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\tab}[6]{$#1$ & #2 & #3 & $#4$ & #5 & #6\\}
\renewcommand{\arraystretch}{1.15}

The next table summarizes the largest partial decay widths for each unstable particles, given in GeV. All of them agrees well within the percent level. We have used here only a single Monte-Carlo generator, MadGraph.

\begin{center}\begin{tabular}{|l|c c| |l|c c|}
  \hline
  Process & MG-FR & MG-ST & Process & MG-FR & MG-ST\\
  \hline \hline
  \tab{t   \,\to\, W^+ \,b     }{1.5608   }{1.5561   }{Z   \,\to\, d \,\bar d}{3.6625e-1}{3.6712e-1}
  \tab{W^+ \,\to\, c   \,\bar s}{6.6807e-1}{6.6830e-1}{h^0 \,\to\, b \,\bar b}{1.6268e-3}{1.6268e-3}
  \tab{H^0 \,\to\, b   \,\bar b}{4.5381e-1}{4.5381e-1}{A^0 \,\to\, b \,\bar b}{4.5479e-1}{4.5479e-1}  
  \tab{H^+ \,\to\, t   \,\bar b}{4.3833e-1}{4.3833e-1}{                }{         }{         }
  \hline \hline
  \tab{\tilde u_1   \,\to\, \tilde\chi_1^+ \,b       }{1.3661   }{1.3661   }{\tilde u_2   \,\to\, \tilde\chi_1^0 \,u      }{1.1373   }{1.1373   }
  \tab{\tilde u_3   \,\to\, \tilde\chi_1^0 \,c       }{1.1373   }{1.1373   }{\tilde u_4   \,\to\, \tilde\chi_1^+ \,s      }{3.5574   }{3.5574   }
  \tab{\tilde u_5   \,\to\, \tilde\chi_1^+ \,d       }{3.5574   }{3.5574   }{\tilde u_6   \,\to\, \tilde\chi_1^+ \,b      }{1.6194   }{1.6194   }
  \tab{\tilde d_1   \,\to\, \tilde\chi_1^- \,t       }{1.6657   }{1.6657   }{\tilde d_2   \,\to\, \tilde\chi_1^0 \,b      }{2.2941e-1}{2.2941e-1}
  \tab{\tilde d_3   \,\to\, \tilde\chi_1^0 \,s       }{2.8196e-1}{2.8196e-1}{\tilde d_4   \,\to\, \tilde\chi_1^0 \,d      }{2.8196e-1}{2.8196e-1}
  \tab{\tilde d_5   \,\to\, \tilde\chi_1^- \,u       }{3.2220   }{3.2220   }{\tilde d_6   \,\to\, \tilde\chi_1^- \,c      }{3.2220   }{3.2220   }
  \tab{\tilde \nu_1 \,\to\, \tilde\chi_1^0 \,\nu_\tau}{1.4545e-1}{1.4545e-1}{\tilde \nu_2 \,\to\, \tilde\chi_1^0 \,\nu_\mu}{1.4654e-1}{1.4654e-1}
  \tab{\tilde \nu_3 \,\to\, \tilde\chi_1^0 \,\nu_e   }{1.4654e-1}{1.4654e-1}{\tilde l_1   \,\to\, \tilde\chi_1^0 \,\tau^- }{1.4833e-1}{1.4833e-1}
  \tab{\tilde l_2   \,\to\, \tilde\chi_1^0 \,e^-     }{2.1612e-1}{2.1612e-1}{\tilde l_3   \,\to\, \tilde\chi_1^0 \,\mu^-  }{2.1612e-1}{2.1612e-1}
  \tab{\tilde l_4   \,\to\, \tilde\chi_1^0 \,\mu^-   }{1.2247e-1}{1.2247e-1}{\tilde l_5   \,\to\, \tilde\chi_1^0 \,e^-    }{1.2247e-1}{1.2247e-1}
  \tab{\tilde l_6   \,\to\, \tilde\chi_1^0 \,\tau^-  }{1.6104e-1}{1.6104e-1}{ }{ }{ }
  \hline \hline
  \tab{\tilde g        \,\to\, \tilde\d_1^\dagger \,b       }{5.5408e-1}{5.5370e-1}{\tilde \chi_2^0 \,\to\, \tilde l_1^-    \,\tau^+}{9.1581e-3}{9.1507e-3}
  \tab{\tilde \chi_3^0 \,\to\, \tilde\chi_1^+     \,W^-     }{5.6624e-1}{5.6460e-1}{\tilde \chi_4^0 \,\to\, \tilde\chi_1^+  \,W^-   }{6.4519e-1}{6.4576e-1}
  \tab{\tilde \chi_1^+ \,\to\, \tilde l_1^+       \,\nu_\tau}{1.5768e-2}{1.5748e-2}{\tilde \chi_2^+ \,\to\, \tilde\chi_2^0  \,W^+   }{7.2945e-1}{7.2998e-1}
  \hline
\end{tabular}\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{\textbf{Production of two Standard Model particles}}
\label{App:SUSYTables2to2SM}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

The tables given in this Appendix contains the production cross sections for two Standard Model particles for various initial states. All the results are given in pb, the partonic center of mass energy is fixed at 1200 GeV or 2000 GeV and we confront the built-in and FeynRules implementations of the MSSM for both MadGraph and CalcHEP, denoted MG-FR, MG-ST, CH-FR and CH-ST. We show only processes for which the cross section is the largest. Again, the complete list of results can be found on the FeynRules webpage.\\

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent{\textbf{Leptonic initial states}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand{\tab}[5]{$#1$ & #2 & #3 & #4 & #5\\}
\begin{center}\begin{tabular}{|l|c c|c c|}
  \hline
  Process & MG-FR & MG-ST & CH-FR & CH-ST\\
  \hline \hline
  \tab{e^+ \,e^- \,\to\, \mu^+    \, \mu^-        }{         }{         }{         }{         }
  \tab{e^+ \,e^- \,\to\, e^+      \, e^-          }{         }{         }{         }{         }
  \tab{e^+ \,e^- \,\to\, \tau^+   \, \tau^-       }{         }{         }{         }{         }
  \tab{e^+ \,e^- \,\to\, \nu_e    \, \bar \nu_e   }{         }{         }{         }{         }
  \hline
\end{tabular}\end{center}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent{\textbf{Quark initial states}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent{\textbf{Gauge boson initial states}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent{\textbf{Other}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\noindent{\textbf{Standalone}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{\textbf{Production of two supersymmetric particles from a leptonic initial state}}
\label{App:SUSYTables2to2SUSYee}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{\textbf{Production of two supersymmetric particles from a quark initial state}}
\label{App:SUSYTables2to2SUSYqq}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{\textbf{Production of two supersymmetric particles through gauge-boson fusion}}
\label{App:SUSYTables2to2SUSYVV}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{\textbf{Production of two supersymmetric particles through other initial states}}
\label{App:SUSYTables2to2SUSYother}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{\textbf{Associated production of two supersymmetric and one Standard Model particle}}
\label{App:SUSYTables2to3}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



